APRICOT: Active Preference Learning and Constraint-Aware Task Planning with LLMs

Home robots performing personalized tasks must adeptly balance user preferences with environmental affordances. We focus on organization tasks within constrained spaces, such as arranging items into a refrigerator, where preferences for placement collide with physical limitations. The robot must infer user preferences based on a small set of demonstrations, which is easier for users to provide than extensively defining all their requirements. While recent works use Large Language Models (LLMs) to learn preferences from user demonstrations, they encounter two fundamental challenges. First, there is inherent ambiguity in interpreting user actions, as multiple preferences can often explain a single observed behavior. Second, not all user preferences are practically feasible due to geometric constraints in the environment. To address these challenges, we introduce APRICOT, a novel approach that merges LLM-based Bayesian active preference learning with constraint-aware task planning. APRICOT refines its generated preferences by actively querying the user and dynamically adapts its plan to respect environmental constraints. We evaluate APRICOT on a dataset of diverse organization tasks and demonstrate its effectiveness in real-world scenarios, showing significant improvements in both preference satisfaction and plan feasibility. The project website is at https://portal-cornell.github.io/apricot/

==> figure_tex/e2e_qualitative.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/e2e_qual_v2.png}
    \vspace{-5mm}
    \captionsetup{width=\textwidth}
    \caption{\textbf{Qualitative Results of Plans for a Hard scenario.} \apricot{} is able to successfully reason about the tension between the space constraints and the user preference (on vegetables and fruits). 
    % Its plan enables the robot to place all objects into the fridge while satisfying the preference.
    \vspace{-2em}}
    \label{fig:e2e_experiment_qual}
\end{figure}

% Have a progress bar that cross out objects not being placed
% Pepsi up
% Vegetable placement

==> figure_tex/task_planner_approach.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/task_planner_approach.png}
    \vspace{-5mm}
    \captionsetup{width=\textwidth}
    \caption{Task Planner Approach}
    \label{fig:task_planner_approach}
\end{figure}

==> input_tex/approach_tex/pref_learning_algo_less-scary.tex <==
\begin{algorithm}[t]
\caption{\apricot{} LLM-based Bayesian Active Preference Learning}
\label{alg:pref_learning}
\begin{algorithmic}
    \State {\bfseries Input:} Demonstrations $\mathcal{D}$, Terminate Function $f_{s_0}$, LLM to generate candidate preferences $P^{\text{gen-pref}}$, LLM to generate questions $P^{\text{gen-q}}$
    \State {\bfseries Output:} Optimal preference $\theta^*$
    \State Generate $N$ candidate preferences: $\theta \sim P^{\text{gen-pref}}(\theta | \mathcal{D})$ 
    \State Initialize uniform prior $P(\theta_i) = \frac{1}{N}$
    %%%%%%%%%%%%%%%
    \State \algcommentlight{While there does not exist a candidate preference that is good enough to approximate the ground-truth preference}
    \State \While {not $f(P(\theta), s_0)$}
    {
        \State Find the best question: $q^* \gets \argmax_{q} H[P(\theta)] - \E_{o} H [P(\theta | q, o)]$
        \State Query user with $q^*$ and gets answer $o_h$
        \State Update prior: $P(\theta) = P(\theta | q=q^*, o=o_h)$
    }
    \State {\bfseries Return} $\xi^*$, $\theta^* \gets \argmax P(\theta)$
\end{algorithmic}
\end{algorithm}

==> input_tex/experiments_tex/overall_results.tex <==
\subsection{Overall Result}
We focus on answering the following questions
\begin{itemize}[leftmargin=*]
    \item \apricot{}'s active preference learning infers preferences that $63.0\%$ of time are consistent with the ground-truth hidden preference in under $3$ queries to a user when being tested on a benchmark dataset with 100 diverse test cases.
    \item \apricot{}'s planner and real robot system generate and execute plans that are $98.0\%$ geometrically feasible and receive an average reward of $0.95/1.00$ when being evaluated on 9 real-world scenarios, placing up to 5 objects into a fridge already with 6 objects.
\end{itemize}

==> input_tex/limitation.tex <==
\section{Limitation}
We highlight key areas for future work:

\textbf{LLM-based Active Preference Learning} The main limitation lies in assuming that one of the candidate preferences is equivalent to the ground-truth preference. 
This assumption allows the terminating conditions to be efficiently computed. 
However, in cases where LLMs hallucinate and only generate incorrect candidate preferences, future work will explore extending our Bayesian framework to allow candidate preferences to be updated based on the user's answers. 

\textbf{Task Planner} The main limitation lies in the decoupling of the preference and geometric feasibility. LLMs struggle when their output must abide by hard constraints. While we try to address this decoupling by replanning using feedback, there is still no guarantee for a correct output. Future work can explore equipping LLMs with tools to improve their geometric reasoning. 

==> input_tex/prompt_files/one_prompt_interactive.tex <==
\definecolor{lightgray}{gray}{0.9}
\definecolor{darkgray}{gray}{0.4}
\definecolor{purple}{rgb}{0.58,0,0.82}

\lstdefinelanguage{plan}{
  sensitive=true,
  morecomment=[l]{//},
}

\lstset{
  language=plan,
  basicstyle=\ttfamily,
  keywordstyle=\color{blue},
  commentstyle=\color{darkgray},
  stringstyle=\color{purple},
  showstringspaces=false,
  columns=fullflexible,
  backgroundcolor=\color{lightgray},
  frame=single,
  breaklines=true,
  breakindent=0pt,
  postbreak=\mbox{{$\hookrightarrow$}\space},
  escapeinside={(*@}{@*)}
}

\begin{lstlisting}
--------- System Message --------
You are a helpful, thoughtful assistant whose task is to infer the user's preference from the demonstrations that the user provides and asking users for yes/no clarification question. 
--------- Instruction --------
  # Input
  You are giving demonstrations, a new initial condition of the fridge that your generated preference will get used at, and chat log of what you have asked so far. 

  ## Demonstrations
  You are given 2 demonstrations that show the before and after when a set of objects gets put into the fridge.  For each demonstration:
  - "Objects that got put away" describes the objects that the user will demonstrate how they would like to put in the fridge.
  - "Initial state of the fridge" describes the objects that are initially in the fridge before the user starts the demonstration. 
  - "Final state of the fridge" describes what the fridge looks like after the demonstration. All the objects in "Objects that got put away" should be in the fridge now. 

  ## New initial state of the fridge
  This is the new initial state that your preference will get used to determine how a new set of objects will get placed into the fridge and satisfy the user's preference.

  ## Objects to put away
  This is the list of object that will get put away in this new initial state of the fridge.

  ## Chat log
  This is a json that contains a history of your thought and your conversation with the user.
  - When the "role" is "thought", this is your internal reasoning about what you were going to do. The user never sees your thought.
  - When the "role" is "assistant", this is the yes/no clarification question that you ask the user about. 
  - When the "role" is "user", this is the yes/no answer that the user provided to your yes/no clarification question.

  ## Can you still ask question?
  There is a maximum number of questions that you can ask. This field will tell you if you can still ask questions or if you must terminate and generate your best guess at the user's preference.

  # Goal
  Your goal is to infer what the user's preference in how the grocery items should be placed into the fridge. You can do this inference by analyzing the demonstrations that the user provide and asking users yes/no clarification questions. Doing this process, you can choose betwwen 2 actions: 
    (1) Ask the user a yes/no clarification question
    (2) Generate the inferred preference and terminate

  # Instructions and useful information
  ## Set up of the fridge
  The fridge can be segmented into 3 shelves (top shelf, middle shelf, bottom shelf); each shelf has 2 sides (left side, right side):
  - left side of the top shelf, right side of the top shelf
  - left side of the middle shelf, right side of the middle shelf
  - left side of the bottom shelf, right side of the bottom shelf

  ## Details about the preferences that you need to output
  A preference is a short paragraph that specifies requirements for each category of grocery items. There must be at least one requirement for each category. The type of requirement for each category can be different. The categories are: "Fruits", "Vegetables", "Juice-and-soft-drinks", "Dairy-Products", and "Condiments".  

  The requirement needs to be one of the following:
  - **Type-1. Specific Locations.** These represent that the object must place at this specific location. The options are: 
    - "left side of top shelf"
    - "right side of top shelf"
    - "left side of middle shelf"
    - "right side of middle shelf"
    - "left side of bottom shelf"
    - "right side of bottom shelf".
  - **Type-2. General Locations.** These are vaguer locations that contain multiple specific locations. The options are:
    - "left side of fridge": which means that the user is ok if the object is placed on "left side of top shelf", "left side of middle shelf", or "left side of bottom shelf"
    - "right side of fridge": which means that the user is ok if the object is placed on "right side of top shelf", "right side of middle shelf", or "right side of bottom shelf"
    - "top shelf": which means that the user is ok if the object is either placed on the "left side of top shelf" or "right side of top shelf"
    - "middle shelf": which means that the user is ok if the object is either placed on the "left side of middle shelf" or "right side of middle shelf"
    - "bottom shelf": which means that the user is ok if the object is either placed on the "left side of bottom shelf" or "right side of bottom shelf"
  - **Type-3. Relative Positions.** The options are: 
    - "<category> must be placed together next to existing <category> regardless of which shelf they are on.": This means that the user only cares that a category of objects are placed together next to existing objects of the same type. The user does not care which specific shelf or which side of the shelf the objects are placed on. For example: "fruits must be placed together next to existing fruits regardless which shelf they are on."
    - "<category> must be placed on the same shelf next to <another category of objects>, and which specific shelf does not matter.": This means that the user only cares that a category of objects are placed together on the same shelf next to another category of objects. It does not matter which specific shelf the objects are on. For example: "fruits must be placed on the same shelf next to condiments, and which specific shelf does not matter."

  In addition to giving specific requirements for each category of grocery items, sometimes you may choose to add additional requirements. The options are:
  - **Type-4. Exception For Attribute**
    - "<category> needs to be placed at <specific location 1>, but <attribute of category> needs to be placed at <specific location 2>.": This means that the user has a different specific requirement for object with a certain attribute compared to the main category. An attribute includes a subcategory of the object, the size/weight of the object, a specific feature of the object, etc. For example, "Dairy product needs to be placed at the right side of top shelf, but cheese needs to be placed at left side of middle shelf." Here, "dairy product" is the main category, and "cheese" is the attribute, which is a specific type of dairy product. Another example is, "Fruits needs to be placed at the left side of middle shelf, but big fruits needs to be placed at right side of bottom shelf." Here, "fruits" is the main category, and "big fruit" is the attribute, which is about the size of the fruit.
  - **Type-5. Conditional On Space**
    - "If there are less than <N> objects at <priminary specific location>, I want <category> to be placed at <priminary specific location>. Else, I want <category> to be placed at <second choice specific location>.": This means that there is a maximum number of objects that can be placed at top choice specific location. If that top choice specific location does not have less than N number of objects, the user wants the a category of objects to be placed at the second choice specific location. For example, "if there are less than 3 objects at the right side of top shelf, I want dairy products to be placed at right side of top shelf. Else, I want dairy products to be placed at left side of middle shelf."

  ## Concrete steps that you must follow
  To successfully determine the user's preference, you must do the following steps.
  ### Step 1: Reasoning about what actions to do
  You can choose between 2 actions: 
  (1) Ask the user a yes/no clarification question
  (2) Generate the inferred preference and terminate

  You must follow these rules when you are deciding what to do:
  - If you are still uncertain about the preference, you should ask an informative yes/no clarification question. 
  - If you are 100% confident about the preference, you can generate what you think the preference is and terminate.

  ### Step 2: Take the action that you decided to do
  You must reply in a valid json format: 
  ```json
  {
    "terminate? (yes/no)": "<you must only reply yes or no>",
    "reasoning": "<you must write down the reasoning behind either why you generated a specific question (if you choose the first action) or why you think the user's preference is what you are generating (if you choose the second action)>",
    "question": "<you must only fill out this string if you chose action (1) ask yes/no clarification question. Otherwise, you must leave this as an empty string.>",
    "preference": "<you must only fill out this string if you chose action (2) generate preference. Otherwise, you must leave this as an empty string.>"
  }
  ```

  #### If you chose (1) Ask the user a yes/no clarification question in Step 3
  You must follow these rules when coming up with questions to ask:
  - You must ask simple yes or no questions. 
  - Your questions cannot ask if the user prefers A or B. However, you can ask if the user prefers A rather than B.
  - Your questions must not be about overall objects or items.You must never ask questions like "Do you prefer to items to be ...?" or "Do you prefer items of the same category ...?" 
  - Your question must be about specifc categories or type of objects. The categories are for example: ["fruits", "vegetables", "dairy product", "condiments", "juice and drinks"]

  Remember that you must reply in a valid json format:
  ```json
  {
    "terminate? (yes/no)": "no",
    "reasoning": "<you must write down the reasoning behind why you generated a specific question (because you choose the first action)",
    "question": "<you must fill out this string because you chose action (1) ask yes/no clarification question.",
    "preference": ""
  }
  ```

  #### If you chose (1) Ask the user a yes/no clarification question in Step 3
  You must follow these rules when generating the preference.
  - You must now terminate so you should answer "yes" under the key "terminate? (yes/no)"
  - Each preference must be in natural language.
  - Each preference must contain at least one placement requirement for each category of objects: "fruits", "vegetables", "drinks", "dairy product", and "condiments".

  Remember that you must reply in a valid json format:
  ```json
  {
    "terminate? (yes/no)": "yes",
    "reasoning": "<you must write down the reasoning behind why you think the user's preference is what you are generating (because you choose the second action)",
    "question": "",
    "preference": "<you must fill out this string with the preference in natural language because you chose action (2) generate preference."
  }
  ```
\end{lstlisting}

==> miscs/authors_list.tex <==
 % The \author macro works with any number of authors. There are two
% commands used to separate the names and addresses of multiple
% authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to
% break the lines. Using \AND forces a line break at that point. So,
% if LaTeX puts 3 of 4 authors names on the first line, and the last
% on the second line, try using \AND instead of \And before the third
% author name.

% NOTE: authors will be visible only in the camera-ready and preprint versions (i.e., when using the option 'final' or 'preprint'). 
% 	For the initial submission the authors will be anonymized.

\author{
Huaxiaoyue Wang$^1$, Nathaniel Chin$^1$, Gonzalo Gonzalez-Pumariega$^1$, Xiangwan Sun$^1$, \\
\bf Neha Sunkara$^1$, Maximus Adrian Pace$^1$, Jeannette Bohg$^2$, Sanjiban Choudhury$^1$
\\$^1$Cornell University, $^2$Stanford University}

% \makeatletter
% \def\thanks#1{\protected@xdef\@thanks{\@thanks \protect\footnotetext{#1}}}
% \makeatother

% \footnote{Correspondence to: Huaxiaoyue Wang, \href{mailto:yukiwang@cs.cornell.edu}{yukiwang@cs.cornell.edu}}

